Multi-Grained Angle Representation for Remote Sensing Object Detection

Arbitrary-oriented object detection (AOOD) plays a significant role for image understanding in remote sensing scenarios. The existing AOOD methods face the challenges of ambiguity and high costs in angle representation. To this end, a multi-grained angle representation (MGAR) method, consisting of coarse-grained angle classification (CAC) and fine-grained angle regression (FAR), is proposed. Specifically, the designed CAC avoids the ambiguity of angle prediction by discrete angular encoding (DAE) and reduces complexity by coarsening the granularity of DAE. Based on CAC, FAR is developed to refine the angle prediction with much lower costs than narrowing the granularity of DAE. Furthermore, an Intersection over Union (IoU) aware FAR-Loss (IFL) is designed to improve accuracy of angle prediction using an adaptive re-weighting mechanism guided by IoU. Extensive experiments are performed on several public remote sensing datasets, which demonstrate the effectiveness of the proposed MGAR. Moreover, experiments on embedded devices demonstrate that the proposed MGAR is also friendly for lightweight deployments.

==> author.tex <==
% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{wanghao.jpg}}]{Hao Wang}
% received the B.E. degree from Beijing
% Institute of Technology. Beijing, China, in 2020.
% He is currently pursuing the M.S. degree with the
% School of Information and Electronics Beijing Institute
% of Technology, Beijing, China. His research
% interest includes object detection and its applications.
% \end{IEEEbiography}

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{liwei.jpg}}]{Wei Li}
% (S'11, M'13, SM'16) received the B.E. degree
% in telecommunications engineering from Xidian
% University, Xi'an, China, in 2007, the M.S. degree in
% information science and technology from Sun Yat-
% Sen University, Guangzhou, China, in 2009, and the
% Ph.D. degree in electrical and computer engineering
% from Mississippi State University, Starkville, MS,
% USA, in 2012. Subsequently, he spent 1 year as a
% Postdoctoral Researcher at the University of California,
% Davis, CA, USA.
% He was a Professor with the College of Information
% Science and Technology at Beijing University of Chemical Technology
% from 2013 to 2019. He is currently a professor with the School of Information
% and Electronics, Beijing Institute of Technology. His research interests include
% hyperspectral image analysis, pattern recognition, and data compression.
% He is currently serving as an Associate Editor for the IEEE Signal
% Processing Letters and the IEEE Journal of Selected Topics in Applied Earth
% Observations and Remote Sensing (JSTARS). He has served as Guest Editor
% for special issue of Journal of Real-Time Image Processing, Remote Sensing,
% and IEEE JSTARS. He received the 2015 Best Reviewer award from IEEE
% Geoscience and Remote Sensing Society (GRSS) for his service for IEEE
% JSTARS and the Outstanding Paper award at IEEE International Workshop
% on Hyperspectral Image and Signal Processing: Evolution in Remote Sensing
% (Whispers), 2019.
% \end{IEEEbiography}

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{huangzhanchao.jpg}}]{Zhanchao Huang}
% received the B.E. degree and
% M.S. degree from Beijing University of Chemical
% Technology, Beijing, China, in 2016 and 2019, respectively.
% He is currently pursuing the Ph.D. degree
% with the School of Information and Electronics,
% Beijing Institute of Technology, Beijing, China. His
% research interests include object detection and its
% applications.
% \end{IEEEbiography}

